THOM: Generating Physically Plausible Hand-Object Meshes From Text

Generating photorealistic 3D hand-object interactions (HOIs) from text is important for applications like robotic grasping and AR/VR content creation. In practice, however, achieving both visual fidelity and physical plausibility remains difficult, as mesh extraction from text-generated Gaussians is inherently ill-posed and the resulting meshes are often unreliable for physics-based optimization. We present THOM, a training-free framework that generates physically plausible 3D HOI meshes directly from text prompts, without requiring template object meshes. THOM follows a two-stage pipeline: it first generates hand and object Gaussians guided by text, and then refines their interaction using physics-based optimization. To enable reliable interaction modeling, we introduce a mesh extraction method with an explicit vertex-to-Gaussian mapping, which enables topology-aware regularization. We further improve physical plausibility through contact-aware optimization and vision-language model (VLM)-guided translation refinement. Extensive experiments show that THOM produces high-quality HOIs with strong text alignment, visual realism, and interaction plausibility.

==> CVPR2026/preamble.tex <==

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}








\usepackage{etoolbox}
\usepackage{booktabs}
\usepackage{amsfonts}
\usepackage{amsmath}
\RequirePackage{amssymb}
\usepackage{dsfont}

\usepackage{mdframed}
\usepackage{bm}
\AtEndPreamble{
    \usepackage[capitalize]{cleveref}
    \crefname{section}{Sec.}{Secs.}
    \Crefname{section}{Section}{Sections}
    \Crefname{table}{Table}{Tables}
    \crefname{table}{Tab.}{Tabs.}
}

\newcommand{\manopose}{\bm{\theta}}
\newcommand{\manobeta}{\bm{\beta}}
\newcommand{\noise}{\epsilon}
\newcommand{\hoiparam}{\mathbf{\psi^{\text{hoi}}}}
\newcommand{\gsmean}{\bm{\mu}}

\usepackage{soul}
\newcommand{\strikecomment}[2]{%
  \st{#1}\ \textcolor{blue}{[Yihalem: #2]}%
}

